Grid HTM: Hierarchical Temporal Memory for Anomaly Detection in Videos

The interest for video anomaly detection systems has gained traction for the past few years. The current approaches use deep learning to perform anomaly detection in videos, but this approach has multiple problems. For starters, deep learning in general has issues with noise, concept drift, explainability, and training data volumes. Additionally, anomaly detection in itself is a complex task and faces challenges such as unknowness, heterogeneity, and class imbalance. Anomaly detection using deep learning is therefore mainly constrained to generative models such as generative adversarial networks and autoencoders due to their unsupervised nature, but even they suffer from general deep learning issues and are hard to train properly. In this paper, we explore the capabilities of the Hierarchical Temporal Memory (HTM) algorithm to perform anomaly detection in videos, as it has favorable properties such as noise tolerance and online learning which combats concept drift. We introduce a novel version of HTM, namely, Grid HTM, which is an HTM-based architecture specifically for anomaly detection in complex videos such as surveillance footage.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> background/background.tex <==
Anomaly detection is often defined as detecting data points that deviate from the general distribution~\cite{anomaly_detection}. Unlike most other problems in deep learning, anomaly detection deals with unpredictable and rare events which makes it hard to apply traditional deep learning for anomaly detection. %Popular approaches therefore often employ generative models, that calculate an anomaly measure using generated or reconstructed data. 
A subset of anomaly detection is smart surveillance~\cite{anomalyvideo}, which is the use of video analysis specifically in surveillance. %Recent developments show that generative models have a high degree of accuracy and are consistently improving.
\par
%However, deep learning has issues which makes it unsuitable for complex anomaly detection in surveillance. 
An issue for deep-learning models in general is that they are susceptible to noise in the dataset~\cite{noise1,noise2}, which leads to decreased model accuracy and poor prediction results. Due to the nature of training deep learning models, they are also in most cases not self-supervised and therefore require constant tuning in order to stay effective on changing data. In addition, they require a lot of data before they can be considered effective, and performance increases logarithmically based on the volume of training data~\cite{deeplearning_dataset}. Deep learning models also suffer from issues with out-of-distribution generalization~\cite{deeplearning_ood_generalization_survey}, where a model might perform great on the dataset it is tested on, but performs poorly when deployed in real life. This could be caused by selection bias in the dataset or when there are differences in the causal structure between the training domain and the deployment domain~\cite{deeplearning_ood}. 
%
Another challenge with deep learning models is that they generally suffer from a lack of explainability~\cite{XAI}. While it is known \emph{how} the models make their decisions, their huge parametric spaces make it unfeasible to know \emph{why} they make those predictions. Combined with the vast potential that deep learning offers in critical sectors such as medicine, makes approaches that offer explainability highly attractive.
\par
The HTM theory~\cite{BAMI} introduces a machine learning algorithm which works on the same principles as the brain and therefore solves some of the issues that deep learning has. \gls*{htm} is considered noise resistant and can perform online learning, meaning that it learns as it observes more data. \gls*{htm} replicates the structure of the neocortex which is made up of cortical regions, which in turn are made up of mini-columns and then neurons.

%(see \autoref{fig:cortical_region}).
%\begin{figure}[htb]
%    \centering
%    \includegraphics[width=\linewidth]{background/cortical_region.eps}
%    \caption{Visualization of a cortical region structure in the neocortex according to \gls*{htm} theory.}
%    \label{fig:cortical_region}
%\end{figure}
%\gls*{htm} neurons are more complex than neurons in deep learning, as visualized in \autoref{fig:neuron_comparison}, and perform learning with Hebbian-like learning.
%\begin{figure}[htb]
%    \centering
%        \begin{subfigure}[t]{\linewidth}
%        \centering
%        \includegraphics[width=0.35\linewidth]{background/neuron_ml.eps}
%        \caption{Deep Learning Neuron.}
%    \end{subfigure}\\
%    \begin{subfigure}[t]{0.35\linewidth}
%        \centering
%        \hspace*{0.5cm}
%        \includegraphics[width=\linewidth]{background/neuron_biological.eps}
%        \caption{Biological Neuron.}
%    \end{subfigure}
%    \hfill
%    \begin{subfigure}[t]{0.55\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{background/neuron_htm.eps}
%        \caption{\gls*{htm} Neuron.}
%    \end{subfigure}
%    \caption{Comparison of neurons.}
%    \label{fig:neuron_comparison}
%\end{figure}
The data in an \gls*{htm} model is represented using a \gls*{sdr}, which is a sparse bit array. An encoder converts real world values into \glspl*{sdr}, and there are currently encoders for numbers, geospatial locations, categories, and dates. %(see \autoref{fig:cyclical_encoder}). 
One of the difficulties with \gls*{htm} is making it work on visual data, where creating a good encoder for visual data is still being researched~\cite{CNN_HTM, eyeencoder, MotionAnomalyDetection}.
The learning mechanism consists of two parts, the \gls*{sp} and the \gls*{tm}. The \gls*{sp} learns to extract semantically important information into output \glspl*{sdr}. The \gls*{tm} learns sequences of patterns of \glspl*{sdr} and forms a prediction in the form of a predictive \gls*{sdr}. 
A research study~\cite{AHMAD2017134} has shown that \gls*{htm} is very capable of performing anomaly detection on low-dimensional data and is able to outperform other anomaly detection methods. However, related works, such as \textcite{MotionAnomalyDetection}, show that \gls*{htm} struggles with higher dimensional data. Therefore, a natural conclusion is that HTM should be applied differently, and that a new type of architecture using HTM should be explored for the purpose of video anomaly detection and surveillance.

%\begin{figure}[htb]
%    \centering
%    \includegraphics[width=\linewidth]{background/cyclical_encoder.eps}
%    \caption{A cyclical data encoder which is encoding Thursday.}
%    \label{fig:cyclical_encoder}
%\end{figure}


==> conclusion/conclusion.tex <==
We presented a novel method to perform anomaly detection in videos. Experiments showed that the proposed Grid HTM can be used for unsupervised anomaly detection in complex videos such as surveillance footage. One of the most important future work would be to create a dataset with videos that are several days long and contain anomalies such as car accidents, jaywalking, and other similar anomalous behaviors.
For Grid HTM, more time can be spent exploring other aggregation functions so that the aggregated anomaly score can be used more efficiently. %One could use deep learning for this purpose or perhaps use another layer of HTM, the possibilities are endless.
Additionally, it would be a big benefit to create an algorithm which can decide the parameters for each cell during the calibration phase. It is also possible to improve explainability and robustness by implementing a measure of certainty for each cell.
%\par
%Depth vision or 3D vision should be experimented with, as the depth information could be valuable for anomaly detection in surveillance. With voxels, this could be used similarly to 2D segmentation, where there could be an extra SDR for each layer of depth in the voxelized 3D image.
\par
Finally, experiments should be performed to validate the possibility of having the TM in each cell grow synapses to neighboring cells in order to solve the issue with unstable anomaly output.
%, which was mentioned in \autoref{sec:stabilizing_anomaly_output}.

==> experiment/experiment.tex <==
As stated earlier, one of the use cases of Grid \gls*{htm} is anomaly detection in surveillance, and we using a video from the VIRAT~\cite{VIRAT} video dataset with long duration and a stationary camera, we demonstrate our system. The video consists of technical anomalies in the form of several segments with sudden frame skips in between. There is also a synthetic anomaly introduced in the form of a frame repeat lasting a couple of seconds, essentially "freezing" time, in order to test whether Grid \gls*{htm} is able to understand how objects should be moving in time.
\par
In this experiment, a segmentation model which can extract classes into their respective SDRs is employed. Meaning that there could be an SDR for cars and an SDR for persons, that are then concatenated before being fed into the system. The segmentation model used is PointRend~\cite{pointrend} with a ResNet101~\cite{resnet} backbone, pretrained on ImageNet~\cite{imagenet}, and implemented using PixelLib~\cite{pixellib}. For the sake of simplicity, this experiment will focus only on the segmentation of cars. While on the topic of segmentation, it is important to mention that the segmentation model is not perfect and that there are cases where objects are misclassified as well as cases where cars repeatedly go above and below the confidence threshold.

%\subsection{Results}
\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{experiment/surveillance_result}
    \caption[Grid HTM Anomaly Score Output]{Anomaly score output from Grid HTM.}
    \label{fig:surveillance_results}
\end{figure}
We can see in \autoref{fig:surveillance_results} that Grid \gls*{htm} is detecting when segments begin and end, however it is not possible to use a threshold value to isolate them, and they also have vastly different anomaly scores compared to each other. This is due to the way the aggregation function works, which means that the anomaly output is dependent on the physical size of the anomaly. It should also be noted that a moving average ($n=200$) was applied to smooth out the anomaly score output, otherwise the graph would be too noisy.

With the aggregation functions presented in this paper in mind, it is safe to conclude that looking at the anomaly score output is meaningless for complex data such as a surveillance video. This however does not mean that Grid \gls*{htm} is completely useless, and this can be observed by looking at the visual output of Grid HTM. The visual output during which the first segment anomaly occurs can be seen in \autoref{fig:surveillance_segment}. Here, it is observed that Grid \gls*{htm} correctly marks the sudden change of cars when the current segment ends and a new segment begins.

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.7\linewidth]{experiment/surveillance_anomaly_1.png}
    \caption[Segment Anomaly]{The first segment anomaly, which is marked with red text,  and the corresponding changes detected by Grid HTM. The numbers beneath each frame represent the relative frame number and the current anomaly score respectively.}
    \label{fig:surveillance_segment}
\end{figure}

%\textbf{Road. }
In the original video, there is a road on which cars regularly drive. By observing the visual output, it becomes evident that after some time Grid \gls*{htm} has mostly learned that behavior and does not report those moving cars as anomalies. This is shown in \autoref{fig:surveillance_road_1}.
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.7\linewidth]{experiment/surveillance_road_1.png}
    \caption[Car Driving Along Main Road]{Visual output when a car is driving along a road.}
    \label{fig:surveillance_road_1}
\end{figure}

%\textbf{Frame Repeat. }
To prove that Grid \gls*{htm} has learned that cars on the road should be moving, it is possible to look at the visual output during the period when the video is repeating the same frame and observe if the architecture marks the cars standing still on the road as anomalies.
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.7\linewidth]{experiment/surveillance_freeze_1.png}
    \caption[Frame Repeat Anomaly]{Anomaly output during the repeating frame, the start of the frame repeat is marked with red text. The blue circle highlights the object of interest.}
    \label{fig:surveillance_freeze_1}
\end{figure}
It can be observed in \autoref{fig:surveillance_freeze_1} that the cars along the main road are not marked as anomalies, but this could be attributed to the fact that there is a crossing there and that cars periodically have to stop at that point to let pedestrians cross.
\par
On the other hand, when looking at the anomaly marked with a blue circle, the car on the road in the parking lot is marked as an anomaly that increases in severity as the time goes on during the frame repeat. The reason why that car causes an anomaly is because, unlike the cars on the main road, a car is rarely observed as standing still at that position.
%\par
To prove that the anomaly was actually directly caused by the repeating frame, and not just due to repeating the anomaly in time, it should be compared to the anomaly output if there was no repeating frame.
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.7\linewidth]{experiment/surveillance_freeze_no_freeze.png}
    \caption[No Frame Repeat Anomaly]{Anomaly output when there is no frame repeating, where it should have repeated is marked in red. The blue circle highlights the object of interest.}
    \label{fig:surveillance_freeze_no_freeze}
\end{figure}
It can be observed in \autoref{fig:surveillance_freeze_no_freeze} that the anomaly output is minor compared to when there was a repeating frame, proving that the anomaly was indeed a product of the repeating frame and that Grid \gls*{htm} was able to learn how objects should be moving in time.
\par
Finally, it is interesting to look at how Grid \gls*{htm} handles the repeating frames without multistep temporal patterns, which is shown in \autoref{fig:surveillance_freeze_no_mtp}.
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.7\linewidth]{experiment/surveillance_freeze_no_mtp.png}
    \caption[Frame Repeat No MTP Anomaly]{Anomaly output during the repeating frame, the start of the frame repeat is marked with red text. The blue circle highlights the object of interest. This time without multistep temporal patterns.}
    \label{fig:surveillance_freeze_no_mtp}
\end{figure}
Unfortunately, simply disabling multistep temporal patterns without adjusting the other \gls*{tm} parameters causes the same car to be marked as an anomaly before and during the frame repeat. In fact, as previously mentioned, disabling multistep temporal patterns causes Grid \gls*{htm} to be less noise tolerant which causes a lot more anomalies to be wrongly detected. This is evident in \autoref{fig:surveillance_freeze_no_mtp}, where a higher number of severe anomalies can be observed compared to previous examples. This also highlights how sensitive \gls*{htm} can be regarding parameters. The working code for Grid HTM and the parameters for the experiments conducted in for this paper can be found on \href{https://github.com/vladim0105/GridHTM}{GitHub}\footnote{\url{https://github.com/vladim0105/GridHTM}}.
%\subsection{Parameters}
%Final list of parameters for reproducibility. As previously mentioned, a moving average ($n=200$) was used to smooth the output graph and make it more readable. The mean was used as the aggregation function due to the complex nature of the data.
%\begin{table}[H]
%    \centering
%    \begin{tabularx}{\linewidth}{@{}XlX@{}}
%        \toprule
%        \textbf{Parameter} & \textbf{Value} & \textbf{Notes}                      \\
%        \midrule
%        sp\_grid\_size     & 32, 32         & Size of each grid                   \\
%        tm\_grid\_size     & 16, 16         & Size of each \gls*{sp} grid output. \\
%        min\_sparsity      & 10             &            %                         \\
%        sparsity           & 15             & Expected %average sparsity           \\
%        temporal\_size     & 15             & Size of the %multistep temporal pattern buffer\\
%        \bottomrule
%    \end{tabularx}
%    \caption{Grid HTM specific parameters}
%    \label{tab:surveillance_grid_htm}
%\end{table}
%\begin{table}[H]
%    \centering
%    \begin{tabularx}{\linewidth}{@{}XlX@{}}
%        \toprule
%        \textbf{Parameter} & \textbf{Value} & %\textbf{Notes}                    \\
%        \midrule
%        inputDimensions    & sp\_grid\_size &            %                       \\
%        columnDimensions   & tm\_grid\_size &            %                       \\
%        potentialPct       & 0.2            &            %                       \\
%        potentialRadius    & 5              &            %                       \\
%        localAreaDensity   & 0.05           &            %                       \\
%        globalInhibition   & True           & Set to %False to enable topology   \\
%        wrapAround         & False          &            %                       \\
%        synPermActiveInc   & 0.01           &            %                       \\
%        synPermInactiveDec & 0.00001                     %                       \\
%        stimulusThreshold  & 3              &            %                       \\
%        boostStrength      & 0              & Causes %instability in empty cells \\
%        \bottomrule
%    \end{tabularx}
%    \caption{SP Parameters}
%    \label{tab:surveillance_sp}
%\end{table}
%\begin{table}[H]
%    \centering
%    \begin{tabularx}{\linewidth}{@{}lXX@{}}
%        \toprule
%        \textbf{Parameter}        & \textbf{Value} & %\textbf{Notes}        \\
%        \midrule
%        columnDimensions          & tm\_grid\_size & Same %as the \gls*{sp} \\
%        predictedSegmentDecrement & 0.001          &     %                  \\
%        permanenceIncrement       & 0.01           &     %                  \\
%        permanenceDecrement       & 0.001          &     %                  \\
%        minThreshold              & 10             &     %                  \\
%        activationThreshold       & 10             &     %                  \\
%        cellsPerColumn            & 32             &     %                  \\
%        \bottomrule
%    \end{tabularx}
%    \caption{TM Parameters}
%    \label{tab:surveillance_tm}
%\end{table}



==> glossary.tex <==
\newacronym{htm}{HTM}{Hierarchical Temporal Memory}
\newacronym{tm}{TM}{Temporal Memory}
\newacronym{sp}{SP}{Spatial Pooler}
\newacronym{sdr}{SDR}{Sparse Distributed Representation}
\newacronym{mlp}{MLP}{Multilayer Perceptron}
\newacronym{relu}{ReLU}{Rectifying Linear Unit}
\newacronym{sgd}{SGD}{Stochastic Gradient Descent}
\newacronym{mse}{MSE}{Mean Squared Error}
\newacronym{cnn}{CNN}{Convolutional Neural Network}
\newacronym{bn}{BN}{Batch Normalization}
\newacronym{rnn}{RNN}{Recurrent Neural Network}
\newacronym{gan}{GAN}{Generative Adversarial Network}
\newacronym{ae}{AE}{Autoencoder}
\newacronym{vae}{VAE}{Variational Autoencoder}
\newacronym{orb}{ORB}{Oriented FAST and Rotated BRIEF}

==> introduction/introduction.tex <==
%\label{sec:introduction}
As the global demand for security and automation increases, many seek to use video anomaly detection systems. In the US alone, the surveillance market is expected to reach $\$23.60$ Billion by 2027~\cite{us_video_stats}. Leveraging modern computer vision, modern anomaly detection systems play an important role in increasing monitoring efficiency and reducing the need for expensive live monitoring. Their use cases can vary from detecting faulty products on an assembly line to detecting car accidents on a highway.
\par
The most important component in video anomaly detection systems is the intelligence behind it. The intelligence ranges from simple on-board algorithms to advanced deep learning models, where the latter has experienced increased popularity in the past few years.
Yet, despite the major progress within the field of deep learning, there are still many tasks where humans outperform models, especially in anomaly detection where the anomalies are often undefined. Deep learning approaches also perform poorly when dealing with noise and concept drift.
\par
The cause for the discrepancy lies in the difference between how humans and machine learning algorithms represent data and learn. Most machine learning algorithms use a dense representation of the data and apply back-propagation in order to learn. Human learning happens in the neocortex, where evidence points to that the neocortex uses a sparse representation and performs Hebbian-style learning. For the latter, there is a growing field of machine learning dedicated to replicating the inner mechanics of the neocortex, namely  \gls*{htm} theory~\cite{BAMI}. This theory outlines its advantages over standard machine learning, such as noise-tolerance and the ability to adapt to changing data.
\par

With the advantages of  \gls*{htm} and the rise of video anomaly detection in mind, a natural question one could pose is whether it is possible to apply  \gls*{htm} for anomaly detection in videos. Combined with a lack of related works, it is this very question that is the motivation behind this paper. In this paper, we therefore propose and evaluate Grid HTM which is a novel expansion of the base HTM algorithm that allows for unsupervised anomaly detection in videos. 



==> methodology/methodology.tex <==
This paper proposes and explores a new type of architecture, named Grid HTM, for anomaly detection in videos using \gls*{htm}, and proposes to use segmentation techniques to simplify the data into an SDR-friendly format. These segmentation techniques could be anything from simple binary thresholding to deep learning instance segmentation. Even keypoint detectors such as \gls*{orb}~\cite{orb_detector} could in theory be applied. When explaining Grid HTM, the examples will be taken from deep learning instance segmentation of cars on a video from the VIRAT~\cite{VIRAT} dataset. An example segmentation is shown in \autoref{fig:example_segmentation}.

%\begin{figure}[htb]
%    \centering
%    \includegraphics[width=.40\linewidth]{methodology/original.png}
%    \includegraphics[width=.40\linewidth]{methodology/car_segmentation.png}
%    \caption[Segmentation Result of Cars]{Segmentation result of cars, which is suited to be used as an SDR. Original frame taken from VIRAT~\cite{VIRAT}.}
%    \label{fig:example_segmentation}
%\end{figure}

\begin{figure}[htb]
    \centering
    %Clean data
    \begin{subfigure}[t]{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{methodology/original.png}
        %\caption{Mean.}

    \end{subfigure}%
    \begin{subfigure}[t]{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{methodology/car_segmentation.png}
        %\caption{Non-zero mean.}
    \end{subfigure}
    \caption[Segmentation Result of Cars]{Segmentation result of cars, which is suited to be used as an SDR. Original frame taken from VIRAT~\cite{VIRAT}.}
    \label{fig:example_segmentation}
\end{figure}



The idea is that the \gls*{sp} will learn to find an optimal general representation of cars. How general this representation is can be configured using the various \gls*{sp} parameters, but ideally they should be set so that different cars will be represented similarly while trucks and motorcycles will be represented differently. An example representation by the SP is shown in \autoref{fig:car_segmentation_sp}.


%\begin{figure}[htb]
%    \centering
%    \includegraphics[width=.40\linewidth]{methodology/car_segmentation.png}
%    \includegraphics[width=.40\linewidth]{methodology/car_segmentation_sp.png}
%    \caption[SDR and SP Representation]{The SDR (left) and its corresponding \gls*{sp} representation (right). Note that the \gls*{sp} is untrained.}
%    \label{fig:car_segmentation_sp}
%\end{figure}

\begin{figure}[htb]
    \centering
    %Clean data
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{methodology/car_segmentation.png}
        %\caption{Mean.}

    \end{subfigure}%
    \hspace{0.5mm}
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{methodology/car_segmentation_sp.png}
        %\caption{Non-zero mean.}
    \end{subfigure}
    \caption[SDR and SP Representation]{The SDR (left) and its corresponding \gls*{sp} representation (right). Note that the \gls*{sp} is untrained.}
    \label{fig:car_segmentation_sp}
\end{figure}


\par
The task of the \gls*{tm} will then be to learn the common patterns that the cars exhibit, their speed, shape, and positioning will be taken into account. Finally, the learning will be set so that new patterns are learned quickly, but forgotten slowly. This will allow the model to quickly learn the norm, even if there is little activity, while still reacting to anomalies. This requires that the input is stationary, in our example this means that the camera is not moving.
\par
It is possible to split different segmentation classes into their respective SDRs. This will give the SP and the TM the ability to learn different things for each of the classes. For instance, if there are two classes "person" and "car", then the TM will learn that it is normal for objects belonging to "person" to be on the sidewalk, while objects belonging to "car" will be marked as anomalous when on the sidewalk.
\par
Ideally, the architecture will have a calibration period spanning several days or weeks, during which the architecture is not performing any anomaly detection, but is just learning the patterns.
\section{Improvements}
%As it currently stands, the current architecture is nearly identical to the one used by
\textcite{MotionAnomalyDetection} tested only the base HTM version and showed that the algorithm cannot handle subtle anomalies, therefore multiple improvements needed to be introduced to increase effectiveness.

\textbf{Invariance. }One issue that becomes evident is the lack of invariance, due to the \gls*{tm} learning the global patterns. Using the example, it learns that it is normal for cars to drive along the road but only in the context of there being cars parked in the parking lot. It is instead desired that the \gls*{tm} learns that it is normal for cars to drive along the road, regardless of whether there are cars in the parking lot.
We proposes a solution based on dividing the encoder output into a grid and have a separate \gls*{sp} and \gls*{tm} for each cell in the grid. The anomaly scores of all the cells are then aggregated into a single anomaly score using an aggregation function.

\textbf{Aggregation Function. } Selecting the correct aggregation function is important because it affects the final anomaly output. For instance, it might be tempting to use the mean of all the anomaly scores as the aggregation function:
\begin{align*}
    X         & :\{x \in \mathbb{R} : x \geq 0\}
    \\
    Anomaly\_Score & =\dfrac{\sum\limits_{x \in X}x}{|X|}
\end{align*}
Where $X$ denotes the set of anomaly scores $x$ from each individual grid.
However, this leads to problems with normalization, meaning that an overall anomaly score of 1 is hard to achieve due to many cells having a zero anomaly score. In fact, it becomes unclear what a high anomaly score is anymore. Using the mean also means that anomalies that take up a lot of space will be weighted higher than anomalies that take up a little space, which might not be desirable.
To solve the aforementioned problem and if the data has little noise, a potential aggregation function could be the non-zero mean:
\begin{align*}
    X         & :\{x \in \mathbb{R} : x > 0\}
    \\
    Anomaly\_Score & =
    \begin{cases}
        \dfrac{\sum\limits_{x \in X}x}{|X|} & \text{if } |X| > 0 
        \\
        \hfil 0                             & \text{otherwise}
    \end{cases}
\end{align*}
Meaning that only the cells with a strictly positive anomaly score, will be contributing to the overall anomaly score which helps solve the aforementioned normalization and weighting problem. On the other hand, the non-zero mean will perform poorly when the architecture is exposed to noisy data which could lead to there always being one or more cells with a high anomaly score.
\begin{figure}[htb]
    \centering
    Noisy data
    \begin{subfigure}[t]{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{methodology/aggr_noisy_mean.png}
        \caption{Mean.}
    \end{subfigure}%
    \begin{subfigure}[t]{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{methodology/aggr_noisy_nzmean.png}
        \caption{Non-zero mean.}
    \end{subfigure}
    \caption[Aggregation Functions on Noise Data]{Aggregation function performance on noisy data.}
    \label{fig:aggr_noisy}
\end{figure}
\begin{figure}[htb]
    \centering
    Clean data
    \begin{subfigure}[t]{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{methodology/aggr_clean_mean.png}
        \caption{Mean.}

    \end{subfigure}%
    \begin{subfigure}[t]{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{methodology/aggr_clean_nzmean.png}
        \caption{Non-zero mean.}
    \end{subfigure}
    \caption[Aggregation Functions on Clean Data]{Aggregation functions performance on clean data.}
    \label{fig:aggr_clean}
\end{figure}
\autoref{fig:aggr_noisy} illustrates the effect of an aggregation function for noisy data, where the non-zero mean is rendered useless due to the noise. On the other hand, \autoref{fig:aggr_clean} shows how the non-zero mean gives a clearer anomaly score when the data is clean. %Especially regarding how, unlike the mean, the non-zero mean has a clearly defined range between 0 and 1.

\textbf{Explainability. } Having the encoder output divided into a grid has the added benefit of introducing explainability into the model. By using Grid \gls*{htm} it is now possible to determine where in the input an anomaly has occurred by simply observing which cell has a high anomaly score.
It is also possible to estimate the number of predictions for each cell which can be used as a measure of certainty, where fewer predictions means higher certainty. Making it possible to measure certainty per cell creates a new source of information which can be used for explainability or robustness purposes.

\textbf{Flexibility and Performance. }
In addition, it is also possible to configure the \gls*{sp} and the \gls*{tm} in each cell independently, giving the architecture increased flexibility and to use a non-uniform grid, meaning that some cells can have different sizes. Last but not least, dividing the frame into smaller cells makes enables it to run each cell in parallel for increased performance.

\textbf{Reviewing Encoder Rules. }
A potential challenge with the grid approach is that the rules for creating a good encoder, may not be respected and therefore should be reviewed:
\begin{itemize}
    \item \textbf{Semantically similar data should result in SDRs with overlapping active bits}. In this example, a car at one position will produce an SDR with a high amount of overlapping bits as another car at a similar position in the input image.
    \item \textbf{The same input should always produce the same SDR}. The segmentation model produces a deterministic output given the same input.
    \item \textbf{The output must have the same dimensionality (total number of bits) for all inputs}. The segmentation model output has a fixed dimensionality.
    \item \textbf{The output should have similar sparsity (similar number of one-bits) for all inputs and have enough one-bits to handle noise and subsampling}. The segmentation model does not respect this. An example is that there can be no cars (zero active bits), one car ($n$ active bits), or two cars ($2n$ active bits), and that this will fluctuate over time.
\end{itemize}
The solution for the last rule is two-fold, and  consists of imposing a soft upper bound and a hard lower bound for the number of active pixels within a cell. The purpose is to lower the variation of number of active pixels, while also containing enough semantic information for the \gls*{htm} to work:
\begin{itemize}
    \item Pick a cell size so that the distribution of number of active pixels is as tight as possible, while containing enough semantic information and also being small enough so that the desired invariance is achieved. The cell size acts as a soft upper bound for the possible number of active pixels.
    \item Create a pattern representing emptiness, where the number of active bits is similar to what can be expected on average when there are cars inside a cell. This acts as a hard lower bound for the number of active pixels.
\end{itemize}
There could be situations where a few pixels are active within a cell, which could happen when a car has just entered a cell, but this is acceptable as long as it does not affect the distribution too much. If it does affect the distribution, which can be the case with noisy data, then an improvement would be to add a minimum sparsity requirement before a cell is considered not empty, e.g. less than 5 active pixels means that the cell is empty.  In the following example, the number of active pixels within a cell centered in the video was used to build the distributions seen in \autoref{fig:num_active_pixels_dist}:
\begin{figure}[htb]
    \centering
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{methodology/active_pixels_dist.eps}
        \caption{Without empty pattern.}
    \end{subfigure}%
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{methodology/active_pixels_dist2.eps}
        \caption{With empty pattern and a minimum sparsity requirement of $5$.}
    \end{subfigure}
    \caption[Distribution of Active Pixels]{Distribution of number of active pixels within a cell of size $12\times 12$.}
    \label{fig:num_active_pixels_dist}
\end{figure}


With a carefully selected empty pattern sparsity, the standard deviation of active pixels was lowered from $\mathbf{3.78}$ to $\mathbf{1.41}$. It is possible to automate this process by developing an algorithm which finds the optimal cell size and empty pattern sparsity which causes the least variation of number of active pixels per cell. This algorithm would run as a part of the calibration process.\par
The visual output resulting from these changes, which is an equally important output as the aggregated anomaly score, can be seen in \autoref{fig:gridhtm_output} (for each cell red means higher anomaly score, green lower anomaly score).
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.7\linewidth]{methodology/htm_grid_output.png}
    \caption[Example Grid HTM Output]{Example Grid \gls*{htm} output and the corresponding input. The color represents the anomaly score for each of the cells, where red means high anomaly score and green means zero anomaly score. Two of the cars are marked as anomalous because they are moving, which is something Grid \gls*{htm} has not seen before during its 300 frame (top right) long lifetime.}
    \label{fig:gridhtm_output}
\end{figure}
Since there are now cells that are observing an empty pattern for a lot of the time in sparse data, boosting is recommended to be turned off, otherwise the \gls*{sp} output for the empty cells would change back and forth in order to adjust the active duty cycle.

\textbf{Stabilizing Anomaly Output. }
%\label{sec:stabilizing_anomaly_output}
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.5\linewidth]{methodology/empty_to_notempty.png}
    \caption[Stabilizing Anomaly Output Visualization 1]{High anomaly score when an empty cell (represented with an empty pattern with a sparsity value of 5) changes to being not empty, as something enters the cell.}
    \label{fig:empty_to_notempty}
\end{figure}
Another issue with the grid based approach is when a car first comes into a cell. The \gls*{tm} in that cell has no way of knowing that a car is about to enter, since it does not see outside its own cell, and therefore the first frame that a car enters a cell will cause a high anomaly output. This is illustrated in \autoref{fig:empty_to_notempty} where it can be observed that this effect causes the anomaly output to needlessly fluctuate. The band-aid solution is to ignore the anomaly score for the frame during which the cell goes from being empty to being not empty, which is illustrated in \autoref{fig:empty_to_notempty_fixed}.
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.5\linewidth]{methodology/empty_to_notempty_fixed.png}
    \caption[Stabilizing Anomaly Output Visualization 2]{The anomaly score is ignored (set to 0) for the frame in which the cell changes state from empty to not empty.}
    \label{fig:empty_to_notempty_fixed}
\end{figure}
A more proper solution could be to allow the \gls*{tm} to grow synapses to the TMs in the neighboring cells, but this is not documented in any research papers and might also hinder invariance.

\textbf{Multistep Temporal Patterns. }
%\label{sec:multistep_temporal_patterns}
Since the \gls*{tm} can only grow segments to cells that were active in the previous timestep, it will struggle to learn temporal patterns across multiple timesteps. This is especially evident in high framerate videos, where an object in motion has a similar representation at timestep $t$ and $t+1$, as an object standing still. 

%\autoref{fig:high_fps} visualizes this phenomenon.
%\begin{figure}[htb]
%    \centering
%    \includegraphics[width=0.3\linewidth]{methodology/high_fps_moving.png}
%    \unskip\ \vrule\
%    \includegraphics[width=0.3\linewidth]{methodology/high_fps_still.png}
%    \caption[Comparison of a Moving Object in a High Framerate Video]{Comparison of a moving object (left) and a still object (right)in a high framerate video. They are very similar and could actually end up being represented identically by the SP.}
%    \label{fig:high_fps}
%\end{figure}

This could cause situations where an object that is supposed to be moving, suddenly stands still, yet the \gls*{tm} will not mark it as an anomaly due to it being stuck in a contextual loop. % (see \autoref{fig:contextual_loop}). 
A contextual loop is when one of the predictions at $t$ becomes true at $t+1$, and then one of the predictions at $t+1$ is almost identical to the state at $t$, which becomes true if the object is not moving, causing the \gls*{tm} to enter the same state that it was in at $t$.
%\begin{figure}[htb]
%    \centering
%    \includegraphics[width=0.7\linewidth]{methodology/context%ual_loop.eps}
%    \caption[Contextual Loop Example]{Example of a contextual %loop.}
%    \label{fig:contextual_loop}
%\end{figure}
A solution is to concatenate the past $n$ \gls*{sp} outputs as input into the TM, which is made possible by keeping a buffer of past \gls*{sp} outputs and shifting its contents out as new \gls*{sp} outputs are inserted. %(see \autoref{fig:mtp}). 
This follows the core idea behind encoding time in addition to the data, which makes time act as a contextual anchor. However, in this case there are no timestamps that are suitable to be used as contextual anchors, so as a replacement, the past observations are encoded instead.
\par
%\begin{figure}[htb]
%    \centering
%    \includegraphics[width=0.45\linewidth]{methodology/temporal_concatenation.eps}
%    \unskip\ \vrule\
%    \includegraphics[width=0.45\linewidth]{methodology/temporal_concatenation_still.eps}
%    \caption[Multistep Temporal Pattern Example]{Example of concatenation with $n=3$ when an object is moving from left to right, compared to when an object is not in motion. It can be observed that the SDRs are vastly different.}
%    \label{fig:mtp}
%\end{figure}
Concatenating past observations together will force the \gls*{tm} input, for when an object is in motion and when an object is still, to be unique. High framerate videos can benefit the most from this, and the effect will be more pronounced for higher values of $n$.
\par
A potential side effect of introducing temporal patterns, is that because the TM is now exposed to multiple frames at once, it will be more tolerant to temporal noise. An example of temporal noise is when an object disappears for a single frame due to falling below the classification threshold of the deep learning segmentation model encoder. The reason for the noise tolerance is that instead of the temporal noise making up the entire input for the TM, it now only makes up $\frac{1}{n}$ of the TM input.

\textbf{Use Cases. }
The most intuitive use case is to use Grid \gls*{htm} for semi-active surveillance, where personnel only have to look at segments containing anomalies, leading to drastically increased efficiency. One example is making it possible to have an entire city be monitored by a few people. This is made possible by making it so that people only have to look at segments that Grid \gls*{htm} has found anomalous, which is what drastically lowers the manpower requirement for active monitoring of the entire city.
